Is Translation All You Need? A Study on Solving Multilingual Tasks with Large Language Models

Large language models (LLMs) have demonstrated multilingual capabilities, yet they are mostly English-centric due to the imbalanced training corpora. While prior works have leveraged this bias to enhance multilingual performance through translation, they have been largely limited to natural language processing (NLP) tasks. In this work, we extend the evaluation to real-world user queries and non-English-centric LLMs, offering a broader examination of multilingual performance. Our key contribution lies in demonstrating that while translation into English can boost the performance of English-centric LLMs on NLP tasks, it is not universally optimal. For culture-related tasks that need deep language understanding, prompting in the native language proves more effective as it better captures the nuances of culture and language. Our experiments expose varied behaviors across LLMs and tasks in the multilingual context, underscoring the need for a more comprehensive approach to multilingual evaluation. Therefore, we call for greater efforts in developing and evaluating LLMs that go beyond English-centric paradigms.

==> latex/sections/discussion.tex <==
\section{General Discussions}
\isaac{no need to be this long, can even remove since this is not a survey/position paper}
In this work, we evaluate LLMs on two types of multilingual tasks: traditional NLP tasks and real user queries. 
The NLP tasks are more likely to rely on universal cognitive abilities, like reasoning and comprehension, rather than specific linguistic knowledge. In contrast, tasks involving real user queries and culture-related questions, discussed in Section \ref{sec:real_query}, necessitate models to possess cultural and language understanding to perform well.
By distinguishing between the two types of tasks, we aim to promote fair and accurate evaluations across diverse linguistic contexts. 

Corresponding to the two types of tasks, multilingual LLMs must develop dual competencies: 1) General Language Skills, which are essential for understanding and engaging with both task types. 
2) Specific Language Skills, which are crucial for tasks demanding an understanding of cultural nuances and linguistic subtleties, such as interpreting culturally specific queries.
By equipping LLMs with these comprehensive skills, we ensure their effectiveness in multilingual contexts, enhancing linguistic adaptability and cultural sensitivity.

The benefits of translation on NLP tasks demonstrate the dominance of English-centric LLMs. 
Despite this, Qwen1.5-72B-Chat and Yi-34B-Chat exhibit strong performance in their native Chinese but do not display similar strengths in other languages. This observation suggests that prompting in native languages could be a more effective strategy than mere translation.
However, reliance on translation emphasizes the difficulties in creating LLMs equally adept at processing a wide range of languages, calling for more efforts toward developing strong multilingual LLMs.


==> latex/tables/main_results.tex <==
\begin{table*}[!ht]
    \centering
    \small
    \begin{tabular}{llccccccc}
    \toprule
        \textbf{Model} & \textbf{Prompt type} & \textbf{MGSM} & \textbf{XCOPA} & \textbf{XNLI} & \textbf{PAWS-X} & \textbf{MKQA} & \textbf{XL-Sum} & \textbf{AVG} \\
        \midrule
        \multirow{7}{*}{ChatGPT} & \nativebasic & 34.4 & 72.3 & 52.2 & 49.7 & 35.4 & 31.9 & 46.0 \\ 
         & \enbasic & 41.1 & 76.1 & 63.0 & 62.0 & 36.5 & \textbf{32.7} & 51.9 \\ 
         & \nativecot & 49.9 & 72.4 & 50.6 & 50.3 & 35.4 & 31.1 & 48.3 \\ 
         & \encot & 61.1 & 78.6 & 56.4 & 61.6 & 42.9 & 29.7 & 55.1 \\ 
         & \xlt & 62.3 & 79.3 & 59.2 & 59.4 & 37.6 & 23.4 & 53.5 \\ 
         & \transg & \textbf{73.9} & \textbf{84.5} & \textbf{60.5} & 67.2 & \textbf{43.8} & 30.3 & \textbf{60.0} \\ 
         & \transn & 61.0 & 79.7 & 59.2 & \textbf{67.5} & 37.2 & 28.3 & 55.5 \\ 
         \midrule
        \multirow{7}{*}{bloomz-7b1} & \nativebasic & 1.3 & 21.4 & 8.3 & - & 7.8 & - & 9.7 \\ 
         & \enbasic & 2.0 & 56.5 & 43.9 & - & 10.6 & - & 28.3 \\ 
         & \nativecot & 1.2 & 20.9 & 8.2 & - & 6.5 & - & 9.2 \\ 
         & \encot & 1.7 & 53.9 & 35.9 & - & 9.3 & - & 25.2 \\ 
         & \xlt & 1.7 & 50.5 & 35.4 & - & 8.0 & - & 23.9 \\ 
         & \transg & \textbf{2.7} & \textbf{63.7} & \textbf{44.3} & - & \textbf{17.2} & - & \textbf{32.0} \\ 
         & \transn & 2.4 & 61.8 & 43.8 & - & 14.7 & - & 30.7 \\ 
        \midrule
        \multirow{7}{*}{Mistral-7B-Instruct} & \nativebasic & 11.2 & 54.2 & 42.8 & 44.6 & 7.8 & 25.9 & 31.1 \\ 
         & \enbasic & 23.8 & 34.9 & 50.2 & 46.9 & 7.0 & 21.6 & 30.7 \\ 
         & \nativecot & 17.0 & 53.8 & 43.4 & 44.3 & 7.8 & 24.6 & 31.8 \\ 
         & \encot & 27.6 & 40.8 & 50.0 & 46.6 & 11.5 & 18.7 & 32.5 \\ 
         & \xlt & 31.8 & \textbf{61.5} & 46.0 & 47.8 & 9.6 & 17.6 & 35.7 \\ 
         & \transg & \textbf{41.3} & 59.2 & \textbf{55.0} & 51.5 & \textbf{17.0} & \textbf{32.8} & \textbf{42.8} \\ 
         & \transn & 31.7 & 54.4 & 53.0 & \textbf{52.4} & 15.5 & 32.2 & 39.9 \\ 
        \midrule
        \multirow{7}{*}{Llama-2-13b-Chat} & \nativebasic & 15.6 & 50.1 & 36.4 & 54.0 & 18.3 & 27.5 & 33.6 \\ 
         & \enbasic & 19.0 & 54.3 & 43.4 & \textbf{59.1} & 20.2 & 31.1 & 37.9 \\ 
         & \nativecot & 18.1 & 50.9 & 35.7 & 54.8 & 15.7 & 27.2 & 33.7 \\ 
         & \encot & 19.9 & 54.5 & 43.7 & 57.6 & 19.8 & 30.2 & 37.6 \\ 
         & \xlt & 22.3 & 56.0 & \textbf{51.4} & 55.7 & 19.0 & 21.2 & 37.6 \\ 
         % & \transg & 39.1 & 71.9 & 46.1 & 58.4 & 33.8 & 35.7 & 47.5 \\ 
         % & \transn & 31.8 & 68.2 & 45.4 & 57.8 & 28.4 & 34.2 & 44.3 \\ 
         & \transg & \textbf{39.1} & \textbf{71.9} & 46.1 & 58.4 & \textbf{33.8} & \textbf{35.7} & \textbf{47.5} \\ 
        & \transn & 31.8 & 68.2 & 45.4 & 57.8 & 28.4 & 34.2 & 44.3 \\
        \midrule
        \multirow{7}{*}{Llama-2-70B-Chat} 
        & \nativebasic & 23.6 & 51.5 & 39.0 & 52.8 & 24.8 & 29.4 & 36.2 \\
        & \enbasic & 28.6 & 55.3 & 46.5 & 60.4 & 24.7 & 31.2 & 40.1 \\
        & \nativecot & 23.5 & 50.5 & 37.9 & 54.9 & 21.9 & 25.8 & 34.5 \\
        & \encot & 30.2 & 61.2 & 45.9 & 64.9 & 31.1 & 30.2 & 42.3 \\
        & \xlt & 32.8 & 58.7 & 52.2 & 55.7 & 26.6 & 17.7 & 38.4 \\
        & \transg & \textbf{53.3} & \textbf{80.9} & \textbf{54.0} & 68.5 & \textbf{39.7} & \textbf{33.8} & \textbf{51.8} \\
        & \transn & 43.8 & 77.1 & 52.2 & \textbf{69.2} & 19.4 & 33.1 & 49.1 \\
        % & \nativebasic & 23.6 & 51.5 & 39.0 & 52.8 & 20.6 & 29.4 & 36.2 \\
        % & \enbasic & 28.6 & 55.3 & 46.5 & 60.4 & 18.4 & 31.2 & 40.1 \\ 
        % & \nativecot & 23.5 & 50.5 & 37.9 & 54.9 & 14.5 & 25.8 & 34.5 \\ 
        % & \encot & 30.2 & 61.2 & 45.9 & 64.9 & \textbf{21.6} & 30.2 & 42.3 \\ 
        % & \xlt & 32.8 & 58.7 & 52.2 & 55.7 & 13.0 & 17.7 & 38.4 \\ 
        % & \transg & \textbf{53.3} & \textbf{80.9} & \textbf{54.0} & 68.5 & 20.5 & \textbf{33.8} & \textbf{51.8} \\ 
        % & \transn & 43.8 & 77.1 & 52.2 & \textbf{69.2} & 19.4 & 33.1 & 49.1 \\ 
    \bottomrule
    \end{tabular}
    \caption{Average scores across different languages (excluding English) for the six benchmarks in zero-shot setting. The results of PAWS-X and XL-Sum for bloomz-7b1 are not considered since it was already pre-trained on these tasks. The best result for each model is in \textbf{bold}.}
    \label{tab:main_NLP}
\end{table*}

% \begin{table*}[!ht]
%     \centering
%     \small
%     \begin{tabular}{llccccccc}
%     \toprule
%         \textbf{Model} & \textbf{Prompt type} & \textbf{MGSM} & \textbf{XCOPA} & \textbf{XNLI} & \textbf{PAWS-X} & \textbf{MKQA} & \textbf{XL-Sum} & \textbf{AVG} \\
%         \midrule
%         \multirow{7}{*}{ChatGPT} & \nativebasic & 34.4 & 72.3 & 52.2 & 49.7 & 35.4 & 31.9 & 46.0 \\ 
%          & \enbasic & 41.1 & 76.1 & 63.0 & 62.0 & 36.5 & \textbf{32.7} & 51.9 \\ 
%          & \nativecot & 49.9 & 72.4 & 50.6 & 50.3 & 35.4 & 31.1 & 48.3 \\ 
%          & \encot & 61.1 & 78.6 & 56.4 & 61.6 & 42.9 & 29.7 & 55.1 \\ 
%          & \xlt & 62.3 & 79.3 & 59.2 & 59.4 & 37.6 & 23.4 & 53.5 \\ 
%          & \transg & \textbf{73.9} & \textbf{84.5} & \textbf{60.5} & 67.2 & \textbf{43.8} & 30.3 & \textbf{60.0} \\ 
%          & \transn & 61.0 & 79.7 & 59.2 & \textbf{67.5} & 37.2 & 28.3 & 55.5 \\ 
%          \midrule
%         \multirow{7}{*}{bloomz-7b1} & \nativebasic & 1.3 & 21.4 & 8.3 & - & 7.8 & - & 9.7 \\ 
%          & \enbasic & 2.0 & 56.5 & 43.9 & - & 10.6 & - & 28.3 \\ 
%          & \nativecot & 1.2 & 20.9 & 8.2 & - & 6.5 & - & 9.2 \\ 
%          & \encot & 1.7 & 53.9 & 35.9 & - & 9.3 & - & 25.2 \\ 
%          & \xlt & 1.7 & 50.5 & 35.4 & - & 8.0 & - & 23.9 \\ 
%          & \transg & \textbf{2.7} & \textbf{63.7} & \textbf{44.3} & - & \textbf{17.2} & - & \textbf{32.0} \\ 
%          & \transn & 2.4 & 61.8 & 43.8 & - & 14.7 & - & 30.7 \\ 
%         \midrule
%         \multirow{7}{*}{Mistral-7B-Instruct-v0.2} & \nativebasic & 11.2 & 54.2 & 42.8 & 44.6 & 7.8 & 25.9 & 31.1 \\ 
%          & \enbasic & 23.8 & 34.9 & 50.2 & 46.9 & 7.0 & 21.6 & 30.7 \\ 
%          & \nativecot & 17.0 & 53.8 & 43.4 & 44.3 & 7.8 & 24.6 & 31.8 \\ 
%          & \encot & 27.6 & 40.8 & 50.0 & 46.6 & 11.5 & 18.7 & 32.5 \\ 
%          & \xlt & 31.8 & \textbf{61.5} & 46.0 & 47.8 & 9.6 & 17.6 & 35.7 \\ 
%          & \transg & \textbf{41.3} & 59.2 & \textbf{55.0} & 51.5 & \textbf{17.0} & \textbf{32.8} & \textbf{42.8} \\ 
%          & \transn & 31.7 & 54.4 & 53.0 & \textbf{52.4} & 15.5 & 32.2 & 39.9 \\ 
%         \midrule
%         \multirow{7}{*}{Llama-2-13b-Chat} & \nativebasic & 15.6 & 50.1 & 36.4 & 54.0 & 18.3 & 27.5 & 33.6 \\ 
%          & \enbasic & 19.0 & 54.3 & 43.4 & \textbf{59.1} & 20.2 & 31.1 & 37.9 \\ 
%          & \nativecot & 18.1 & 50.9 & 35.7 & 54.8 & 15.7 & 27.2 & 33.7 \\ 
%          & \encot & 19.9 & 54.5 & 43.7 & 57.6 & 19.8 & 30.2 & 37.6 \\ 
%          & \xlt & 22.3 & 56.0 & \textbf{51.4} & 55.7 & 19.0 & 21.2 & 37.6 \\ 
%          % & \transg & 39.1 & 71.9 & 46.1 & 58.4 & 33.8 & 35.7 & 47.5 \\ 
%          % & \transn & 31.8 & 68.2 & 45.4 & 57.8 & 28.4 & 34.2 & 44.3 \\ 
%          & \transg & \textbf{39.1} & \textbf{71.9} & 46.1 & 58.4 & \textbf{33.8} & \textbf{35.7} & \textbf{47.5} \\ 
%         & \transn & 31.8 & 68.2 & 45.4 & 57.8 & 28.4 & 34.2 & 44.3 \\
%         \midrule
%         \multirow{7}{*}{Llama-2-70B-Chat-AWQ} 
%         & \nativebasic & 23.6 & 51.5 & 39.0 & 52.8 & 24.8 & 29.4 & 36.2 \\
%         & \enbasic & 28.6 & 55.3 & 46.5 & 60.4 & 24.7 & 31.2 & 40.1 \\
%         & \nativecot & 23.5 & 50.5 & 37.9 & 54.9 & 21.9 & 25.8 & 34.5 \\
%         & \encot & 30.2 & 61.2 & 45.9 & 64.9 & 31.1 & 30.2 & 42.3 \\
%         & \xlt & 32.8 & 58.7 & 52.2 & 55.7 & 26.6 & 17.7 & 38.4 \\
%         & \transg & \textbf{53.3} & \textbf{80.9} & \textbf{54.0} & 68.5 & \textbf{39.7} & \textbf{33.8} & \textbf{51.8} \\
%         & \transn & 43.8 & 77.1 & 52.2 & \textbf{69.2} & 19.4 & 33.1 & 49.1 \\
%         % & \nativebasic & 23.6 & 51.5 & 39.0 & 52.8 & 20.6 & 29.4 & 36.2 \\
%         % & \enbasic & 28.6 & 55.3 & 46.5 & 60.4 & 18.4 & 31.2 & 40.1 \\ 
%         % & \nativecot & 23.5 & 50.5 & 37.9 & 54.9 & 14.5 & 25.8 & 34.5 \\ 
%         % & \encot & 30.2 & 61.2 & 45.9 & 64.9 & \textbf{21.6} & 30.2 & 42.3 \\ 
%         % & \xlt & 32.8 & 58.7 & 52.2 & 55.7 & 13.0 & 17.7 & 38.4 \\ 
%         % & \transg & \textbf{53.3} & \textbf{80.9} & \textbf{54.0} & 68.5 & 20.5 & \textbf{33.8} & \textbf{51.8} \\ 
%         % & \transn & 43.8 & 77.1 & 52.2 & \textbf{69.2} & 19.4 & 33.1 & 49.1 \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{Average scores across different languages (excluding English) for the six benchmarks in zero-shot setting. The results of PAWS-X and XL-Sum for bloomz-7b1 are not considered since it was already pre-trained on these tasks. The best result for each model is in \textbf{bold}.}
%     \label{tab:main_NLP}
% \end{table*}


% \begin{table*}[!ht]
%     \label{table:main_results}
%     \centering
%     \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
%     
%         model & prompt\_type & mgsm & xcopa & xnli & paws-x & MKQA & XL-SUM & Average \\ 
%         chatgpt-1106 & basic & 41.1\% & 77.4\% & 63.0\% & 62.0\% & 36.5\% & 32.7\% & 52.1\% \\ 
%         EN-CoT & 61.1\% & 79.7\% & 56.4\% & 61.6\% & 42.9\% & 29.7\% & 55.2\% & ~ \\ 
%         Translate\_test\_google & 73.9\% & 85.1\% & 60.5\% & 67.2\% & 43.8\% & 30.3\% & 60.1\% & ~ \\ 
%         Translate\_test\_nllb & 61.0\% & 80.3\% & 59.2\% & 67.5\% & 37.2\% & 28.3\% & 55.6\% & ~ \\ 
%     \end{tabular}
% \end{table*}

% \begin{table*}[ht]
% \small
% \centering
% \begin{tabular}{l|l|llllll|l}
% 
% Model          & Prompt Type            & MGSM  & XCOPA & XNLI & PAWS-X & MKQA & XL-SUM & Average \\ 

% \end{tabular}
% \caption{Performance of different models on various benchmarks}
% \label{table:performance}
% \end{table*}
